A Case Study on Visualizing Large Spatial Datasets in a Web-based Map Viewer

Lately, many companies are using Mobile Workforce Management technologies combined with information collected by sensors from mobile devices in order to improve their business processes. Even for small companies, the information that needs to be handled grows at a high rate, and most of the data collected have a geographic dimension. Being able to visualize this data in real-time within a map viewer is a very important deal for these companies. In this paper we focus on this topic, presenting a case study on visualizing large spatial datasets. Particularly, since most of the Mobile Workforce Management software is web-based, we propose a solution suitable for this environment.

==> out <==
pdflatex -shell-escape main.tex
This is pdfTeX, Version 3.14159265-2.6-1.40.20 (TeX Live 2019/Arch Linux) (preloaded format=pdflatex)
 \write18 enabled.
entering extended mode
(./main.tex
LaTeX2e <2019-10-01> patch level 1
(./llncs.cls
Document Class: llncs 2018/03/10 v2.20 
 LaTeX document class for Lecture Notes in Computer Science
(/usr/share/texmf-dist/tex/latex/base/article.cls
Document Class: article 2019/08/27 v1.4j Standard LaTeX document class
(/usr/share/texmf-dist/tex/latex/base/size10.clo))
(/usr/share/texmf-dist/tex/latex/tools/multicol.sty)
(/usr/share/texmf-dist/tex/latex/oberdiek/aliascnt.sty)) (./_init.tex
(/usr/share/texmf-dist/tex/latex/cmap/cmap.sty)
(/usr/share/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/share/texmf-dist/tex/generic/oberdiek/soulutf8.sty
(/usr/share/texmf-dist/tex/latex/soul/soul.sty)
(/usr/share/texmf-dist/tex/generic/oberdiek/infwarerr.sty)
(/usr/share/texmf-dist/tex/generic/oberdiek/etexcmds.sty
(/usr/share/texmf-dist/tex/generic/oberdiek/ifluatex.sty)))
(/usr/share/texmf-dist/tex/latex/graphics/color.sty
(/usr/share/texmf-dist/tex/latex/graphics-cfg/color.cfg)
(/usr/share/texmf-dist/tex/latex/graphics-def/pdftex.def))
(/usr/share/texmf-dist/tex/latex/csquotes/csquotes.sty
(/usr/share/texmf-dist/tex/latex/etoolbox/etoolbox.sty)
(/usr/share/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/share/texmf-dist/tex/latex/csquotes/csquotes.def)
(/usr/share/texmf-dist/tex/latex/csquotes/csquotes.cfg))
(/usr/share/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/share/texmf-dist/tex/generic/oberdiek/hobsub-hyperref.sty
(/usr/share/texmf-dist/tex/generic/oberdiek/hobsub-generic.sty))
(/usr/share/texmf-dist/tex/generic/ifxetex/ifxetex.sty)
(/usr/share/texmf-dist/tex/latex/oberdiek/auxhook.sty)
(/usr/share/texmf-dist/tex/latex/oberdiek/kvoptions.sty)
(/usr/share/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/share/texmf-dist/tex/latex/latexconfig/hyperref.cfg)
(/usr/share/texmf-dist/tex/latex/url/url.sty))
(/usr/share/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/share/texmf-dist/tex/latex/oberdiek/rerunfilecheck.sty))
(/usr/share/texmf-dist/tex/latex/listings/listings.sty
(/usr/share/texmf-dist/tex/latex/listings/lstmisc.sty)
(/usr/share/texmf-dist/tex/latex/listings/listings.cfg))
(/usr/share/texmf-dist/tex/latex/breakurl/breakurl.sty
(/usr/share/texmf-dist/tex/latex/xkeyval/xkeyval.sty
(/usr/share/texmf-dist/tex/generic/xkeyval/xkeyval.tex
(/usr/share/texmf-dist/tex/generic/xkeyval/xkvutils.tex)))

Package breakurl Warning: You are using breakurl while processing via pdflatex.

(breakurl)                \burl will be just a synonym of \url.
(breakurl)                 on input line 48.

) (/usr/share/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/share/texmf-dist/tex/latex/booktabs/booktabs.sty)
(/usr/share/texmf-dist/tex/latex/base/makeidx.sty)
(/usr/share/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/share/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/share/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/share/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)))
(/usr/share/texmf-dist/tex/latex/caption/caption.sty
(/usr/share/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unsupported document class (or package) detected,
(caption)                usage of the caption package is not recommended.
See the caption package documentation for explanation.

) (/usr/share/texmf-dist/tex/latex/caption/subcaption.sty)
(/usr/share/texmf-dist/tex/latex/paralist/paralist.sty)
(/usr/share/texmf-dist/tex/latex/cite/cite.sty)
(/usr/share/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/share/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/share/texmf-dist/tex/latex/pdfcomment/pdfcomment.sty
(/usr/share/texmf-dist/tex/latex/datetime2/datetime2.sty
(/usr/share/texmf-dist/tex/latex/tracklang/tracklang.sty
(/usr/share/texmf-dist/tex/generic/tracklang/tracklang.tex)))
(/usr/share/texmf-dist/tex/latex/oberdiek/zref-savepos.sty
(/usr/share/texmf-dist/tex/latex/oberdiek/zref-base.sty))
(/usr/share/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/share/texmf-dist/tex/latex/tools/calc.sty)
(/usr/share/texmf-dist/tex/latex/marginnote/marginnote.sty)
(/usr/share/texmf-dist/tex/latex/soulpos/soulpos.sty)

Package hyperref Warning: Option `pdftex' has already been used,
(hyperref)                setting the option has no effect on input line 1369.

) (/usr/share/texmf-dist/tex/latex/oberdiek/hypcap.sty)
(/usr/share/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/share/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/share/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/share/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/share/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/share/texmf-dist/tex/latex/cleveref/cleveref.sty))

Package csquotes Warning: No multilingual support.
(csquotes)                Cannot enable multilingual quotes on input line 5.

(./main.aux) (/usr/share/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/share/texmf-dist/tex/latex/oberdiek/epstopdf-base.sty
(/usr/share/texmf-dist/tex/latex/oberdiek/grfext.sty)
(/usr/share/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/share/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/share/texmf-dist/tex/generic/oberdiek/gettitlestring.sty))<<ot1.cmap>><<o
ml.cmap>><<oms.cmap>><<omx.cmap>><<ot1tt.cmap>>

LaTeX Font Warning: Font shape `OMS/cmtt/m/n' undefined
(Font)              using `OMS/cmsy/m/n' instead
(Font)              for symbol `textbraceleft' on input line 24.

(./section/01-motivation.tex [1{/var/lib/texmf/fonts/map/pdftex/updmap/pdftex.m
ap}]) (./section/02-background.tex [2] (./code/event.json) [3 <./figures/01_Gen
eral-eps-converted-to.pdf>]
Underfull \vbox (badness 5175) has occurred while \output is active [4 <./figur
es/03_Querying-eps-converted-to.pdf>]

LaTeX Warning: Command \textordmasculine invalid in math mode on input line 38.


) (./section/03-objectives.tex [5]) (./section/04-experiments.tex [6 <./figures
/timedistribution-eps-converted-to.pdf> <./figures/spatialdistribution_colored_
cropped.png (PNG copy)>]) (./section/05-conclusions.tex
Underfull \vbox (badness 2221) has occurred while \output is active [7 <./resul
ts/RQ1.pdf>]) (./main.bbl) [8] (./main.aux
* soulpos - computing points - it may take a few seconds * (./main.upa))

LaTeX Font Warning: Some font shapes were not available, defaults substituted.

 )
(see the transcript file for additional information)</usr/share/texmf-dist/font
s/type1/public/amsfonts/cm/cmbx10.pfb></usr/share/texmf-dist/fonts/type1/public
/amsfonts/cm/cmbx12.pfb></usr/share/texmf-dist/fonts/type1/public/amsfonts/cm/c
mbx9.pfb></usr/share/texmf-dist/fonts/type1/public/amsfonts/cm/cmex10.pfb></usr
/share/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi10.pfb></usr/share/texmf-d
ist/fonts/type1/public/amsfonts/cm/cmmi6.pfb></usr/share/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmib10.pfb></usr/share/texmf-dist/fonts/type1/public/amsfo
nts/cm/cmr10.pfb></usr/share/texmf-dist/fonts/type1/public/amsfonts/cm/cmr6.pfb
></usr/share/texmf-dist/fonts/type1/public/amsfonts/cm/cmr7.pfb></usr/share/tex
mf-dist/fonts/type1/public/amsfonts/cm/cmr9.pfb></usr/share/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmsy10.pfb></usr/share/texmf-dist/fonts/type1/public/ams
fonts/cm/cmsy7.pfb></usr/share/texmf-dist/fonts/type1/public/amsfonts/cm/cmsy9.
pfb></usr/share/texmf-dist/fonts/type1/public/amsfonts/cm/cmti10.pfb></usr/shar
e/texmf-dist/fonts/type1/public/amsfonts/cm/cmtt10.pfb></usr/share/texmf-dist/f
onts/type1/public/amsfonts/cm/cmtt9.pfb></usr/share/texmf-dist/fonts/type1/publ
ic/tex-gyre/qhvr.pfb>
Output written on main.pdf (8 pages, 1075098 bytes).
Transcript written on main.log.
bibtex main.aux
This is BibTeX, Version 0.99d (TeX Live 2019/Arch Linux)
The top-level auxiliary file: main.aux
The style file: splncs03.bst
Database file #1: library.bib
pdflatex -shell-escape main.tex
This is pdfTeX, Version 3.14159265-2.6-1.40.20 (TeX Live 2019/Arch Linux) (preloaded format=pdflatex)
 \write18 enabled.
entering extended mode
(./main.tex
LaTeX2e <2019-10-01> patch level 1
(./llncs.cls
Document Class: llncs 2018/03/10 v2.20 
 LaTeX document class for Lecture Notes in Computer Science
(/usr/share/texmf-dist/tex/latex/base/article.cls
Document Class: article 2019/08/27 v1.4j Standard LaTeX document class
(/usr/share/texmf-dist/tex/latex/base/size10.clo))
(/usr/share/texmf-dist/tex/latex/tools/multicol.sty)
(/usr/share/texmf-dist/tex/latex/oberdiek/aliascnt.sty)) (./_init.tex
(/usr/share/texmf-dist/tex/latex/cmap/cmap.sty)
(/usr/share/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/share/texmf-dist/tex/generic/oberdiek/soulutf8.sty
(/usr/share/texmf-dist/tex/latex/soul/soul.sty)
(/usr/share/texmf-dist/tex/generic/oberdiek/infwarerr.sty)
(/usr/share/texmf-dist/tex/generic/oberdiek/etexcmds.sty
(/usr/share/texmf-dist/tex/generic/oberdiek/ifluatex.sty)))
(/usr/share/texmf-dist/tex/latex/graphics/color.sty
(/usr/share/texmf-dist/tex/latex/graphics-cfg/color.cfg)
(/usr/share/texmf-dist/tex/latex/graphics-def/pdftex.def))
(/usr/share/texmf-dist/tex/latex/csquotes/csquotes.sty
(/usr/share/texmf-dist/tex/latex/etoolbox/etoolbox.sty)
(/usr/share/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/share/texmf-dist/tex/latex/csquotes/csquotes.def)
(/usr/share/texmf-dist/tex/latex/csquotes/csquotes.cfg))
(/usr/share/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/share/texmf-dist/tex/generic/oberdiek/hobsub-hyperref.sty
(/usr/share/texmf-dist/tex/generic/oberdiek/hobsub-generic.sty))
(/usr/share/texmf-dist/tex/generic/ifxetex/ifxetex.sty)
(/usr/share/texmf-dist/tex/latex/oberdiek/auxhook.sty)
(/usr/share/texmf-dist/tex/latex/oberdiek/kvoptions.sty)
(/usr/share/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/share/texmf-dist/tex/latex/latexconfig/hyperref.cfg)
(/usr/share/texmf-dist/tex/latex/url/url.sty))
(/usr/share/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/share/texmf-dist/tex/latex/oberdiek/rerunfilecheck.sty))
(/usr/share/texmf-dist/tex/latex/listings/listings.sty
(/usr/share/texmf-dist/tex/latex/listings/lstmisc.sty)
(/usr/share/texmf-dist/tex/latex/listings/listings.cfg))
(/usr/share/texmf-dist/tex/latex/breakurl/breakurl.sty
(/usr/share/texmf-dist/tex/latex/xkeyval/xkeyval.sty
(/usr/share/texmf-dist/tex/generic/xkeyval/xkeyval.tex
(/usr/share/texmf-dist/tex/generic/xkeyval/xkvutils.tex)))

Package breakurl Warning: You are using breakurl while processing via pdflatex.

(breakurl)                \burl will be just a synonym of \url.
(breakurl)                 on input line 48.

) (/usr/share/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/share/texmf-dist/tex/latex/booktabs/booktabs.sty)
(/usr/share/texmf-dist/tex/latex/base/makeidx.sty)
(/usr/share/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/share/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/share/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/share/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)))
(/usr/share/texmf-dist/tex/latex/caption/caption.sty
(/usr/share/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unsupported document class (or package) detected,
(caption)                usage of the caption package is not recommended.
See the caption package documentation for explanation.

) (/usr/share/texmf-dist/tex/latex/caption/subcaption.sty)
(/usr/share/texmf-dist/tex/latex/paralist/paralist.sty)
(/usr/share/texmf-dist/tex/latex/cite/cite.sty)
(/usr/share/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/share/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/share/texmf-dist/tex/latex/pdfcomment/pdfcomment.sty
(/usr/share/texmf-dist/tex/latex/datetime2/datetime2.sty
(/usr/share/texmf-dist/tex/latex/tracklang/tracklang.sty
(/usr/share/texmf-dist/tex/generic/tracklang/tracklang.tex)))
(/usr/share/texmf-dist/tex/latex/oberdiek/zref-savepos.sty
(/usr/share/texmf-dist/tex/latex/oberdiek/zref-base.sty))
(/usr/share/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/share/texmf-dist/tex/latex/tools/calc.sty)
(/usr/share/texmf-dist/tex/latex/marginnote/marginnote.sty)
(/usr/share/texmf-dist/tex/latex/soulpos/soulpos.sty)

Package hyperref Warning: Option `pdftex' has already been used,
(hyperref)                setting the option has no effect on input line 1369.

) (/usr/share/texmf-dist/tex/latex/oberdiek/hypcap.sty)
(/usr/share/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/share/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/share/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/share/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/share/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/share/texmf-dist/tex/latex/cleveref/cleveref.sty))

Package csquotes Warning: No multilingual support.
(csquotes)                Cannot enable multilingual quotes on input line 5.

(./main.aux) (/usr/share/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/share/texmf-dist/tex/latex/oberdiek/epstopdf-base.sty
(/usr/share/texmf-dist/tex/latex/oberdiek/grfext.sty)
(/usr/share/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/share/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/share/texmf-dist/tex/generic/oberdiek/gettitlestring.sty))<<ot1.cmap>><<o
ml.cmap>><<oms.cmap>><<omx.cmap>><<ot1tt.cmap>>

LaTeX Font Warning: Font shape `OMS/cmtt/m/n' undefined
(Font)              using `OMS/cmsy/m/n' instead
(Font)              for symbol `textbraceleft' on input line 24.

(./section/01-motivation.tex [1{/var/lib/texmf/fonts/map/pdftex/updmap/pdftex.m
ap}]) (./section/02-background.tex [2] (./code/event.json) [3 <./figures/01_Gen
eral-eps-converted-to.pdf>]
Underfull \vbox (badness 5175) has occurred while \output is active [4 <./figur
es/03_Querying-eps-converted-to.pdf>]

LaTeX Warning: Command \textordmasculine invalid in math mode on input line 38.


) (./section/03-objectives.tex [5]) (./section/04-experiments.tex [6 <./figures
/timedistribution-eps-converted-to.pdf> <./figures/spatialdistribution_colored_
cropped.png (PNG copy)>]) (./section/05-conclusions.tex
Underfull \vbox (badness 2221) has occurred while \output is active [7 <./resul
ts/RQ1.pdf>]) (./main.bbl) [8] (./main.aux
* soulpos - computing points - it may take a few seconds * (./main.upa))

LaTeX Font Warning: Some font shapes were not available, defaults substituted.

 )
(see the transcript file for additional information)</usr/share/texmf-dist/font
s/type1/public/amsfonts/cm/cmbx10.pfb></usr/share/texmf-dist/fonts/type1/public
/amsfonts/cm/cmbx12.pfb></usr/share/texmf-dist/fonts/type1/public/amsfonts/cm/c
mbx9.pfb></usr/share/texmf-dist/fonts/type1/public/amsfonts/cm/cmex10.pfb></usr
/share/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi10.pfb></usr/share/texmf-d
ist/fonts/type1/public/amsfonts/cm/cmmi6.pfb></usr/share/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmib10.pfb></usr/share/texmf-dist/fonts/type1/public/amsfo
nts/cm/cmr10.pfb></usr/share/texmf-dist/fonts/type1/public/amsfonts/cm/cmr6.pfb
></usr/share/texmf-dist/fonts/type1/public/amsfonts/cm/cmr7.pfb></usr/share/tex
mf-dist/fonts/type1/public/amsfonts/cm/cmr9.pfb></usr/share/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmsy10.pfb></usr/share/texmf-dist/fonts/type1/public/ams
fonts/cm/cmsy7.pfb></usr/share/texmf-dist/fonts/type1/public/amsfonts/cm/cmsy9.
pfb></usr/share/texmf-dist/fonts/type1/public/amsfonts/cm/cmti10.pfb></usr/shar
e/texmf-dist/fonts/type1/public/amsfonts/cm/cmtt10.pfb></usr/share/texmf-dist/f
onts/type1/public/amsfonts/cm/cmtt9.pfb></usr/share/texmf-dist/fonts/type1/publ
ic/tex-gyre/qhvr.pfb>
Output written on main.pdf (8 pages, 1075098 bytes).
Transcript written on main.log.
pdflatex -shell-escape main.tex
This is pdfTeX, Version 3.14159265-2.6-1.40.20 (TeX Live 2019/Arch Linux) (preloaded format=pdflatex)
 \write18 enabled.
entering extended mode
(./main.tex
LaTeX2e <2019-10-01> patch level 1
(./llncs.cls
Document Class: llncs 2018/03/10 v2.20 
 LaTeX document class for Lecture Notes in Computer Science
(/usr/share/texmf-dist/tex/latex/base/article.cls
Document Class: article 2019/08/27 v1.4j Standard LaTeX document class
(/usr/share/texmf-dist/tex/latex/base/size10.clo))
(/usr/share/texmf-dist/tex/latex/tools/multicol.sty)
(/usr/share/texmf-dist/tex/latex/oberdiek/aliascnt.sty)) (./_init.tex
(/usr/share/texmf-dist/tex/latex/cmap/cmap.sty)
(/usr/share/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/share/texmf-dist/tex/generic/oberdiek/soulutf8.sty
(/usr/share/texmf-dist/tex/latex/soul/soul.sty)
(/usr/share/texmf-dist/tex/generic/oberdiek/infwarerr.sty)
(/usr/share/texmf-dist/tex/generic/oberdiek/etexcmds.sty
(/usr/share/texmf-dist/tex/generic/oberdiek/ifluatex.sty)))
(/usr/share/texmf-dist/tex/latex/graphics/color.sty
(/usr/share/texmf-dist/tex/latex/graphics-cfg/color.cfg)
(/usr/share/texmf-dist/tex/latex/graphics-def/pdftex.def))
(/usr/share/texmf-dist/tex/latex/csquotes/csquotes.sty
(/usr/share/texmf-dist/tex/latex/etoolbox/etoolbox.sty)
(/usr/share/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/share/texmf-dist/tex/latex/csquotes/csquotes.def)
(/usr/share/texmf-dist/tex/latex/csquotes/csquotes.cfg))
(/usr/share/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/share/texmf-dist/tex/generic/oberdiek/hobsub-hyperref.sty
(/usr/share/texmf-dist/tex/generic/oberdiek/hobsub-generic.sty))
(/usr/share/texmf-dist/tex/generic/ifxetex/ifxetex.sty)
(/usr/share/texmf-dist/tex/latex/oberdiek/auxhook.sty)
(/usr/share/texmf-dist/tex/latex/oberdiek/kvoptions.sty)
(/usr/share/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/share/texmf-dist/tex/latex/latexconfig/hyperref.cfg)
(/usr/share/texmf-dist/tex/latex/url/url.sty))
(/usr/share/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/share/texmf-dist/tex/latex/oberdiek/rerunfilecheck.sty))
(/usr/share/texmf-dist/tex/latex/listings/listings.sty
(/usr/share/texmf-dist/tex/latex/listings/lstmisc.sty)
(/usr/share/texmf-dist/tex/latex/listings/listings.cfg))
(/usr/share/texmf-dist/tex/latex/breakurl/breakurl.sty
(/usr/share/texmf-dist/tex/latex/xkeyval/xkeyval.sty
(/usr/share/texmf-dist/tex/generic/xkeyval/xkeyval.tex
(/usr/share/texmf-dist/tex/generic/xkeyval/xkvutils.tex)))

Package breakurl Warning: You are using breakurl while processing via pdflatex.

(breakurl)                \burl will be just a synonym of \url.
(breakurl)                 on input line 48.

) (/usr/share/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/share/texmf-dist/tex/latex/booktabs/booktabs.sty)
(/usr/share/texmf-dist/tex/latex/base/makeidx.sty)
(/usr/share/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/share/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/share/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/share/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)))
(/usr/share/texmf-dist/tex/latex/caption/caption.sty
(/usr/share/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unsupported document class (or package) detected,
(caption)                usage of the caption package is not recommended.
See the caption package documentation for explanation.

) (/usr/share/texmf-dist/tex/latex/caption/subcaption.sty)
(/usr/share/texmf-dist/tex/latex/paralist/paralist.sty)
(/usr/share/texmf-dist/tex/latex/cite/cite.sty)
(/usr/share/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/share/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/share/texmf-dist/tex/latex/pdfcomment/pdfcomment.sty
(/usr/share/texmf-dist/tex/latex/datetime2/datetime2.sty
(/usr/share/texmf-dist/tex/latex/tracklang/tracklang.sty
(/usr/share/texmf-dist/tex/generic/tracklang/tracklang.tex)))
(/usr/share/texmf-dist/tex/latex/oberdiek/zref-savepos.sty
(/usr/share/texmf-dist/tex/latex/oberdiek/zref-base.sty))
(/usr/share/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/share/texmf-dist/tex/latex/tools/calc.sty)
(/usr/share/texmf-dist/tex/latex/marginnote/marginnote.sty)
(/usr/share/texmf-dist/tex/latex/soulpos/soulpos.sty)

Package hyperref Warning: Option `pdftex' has already been used,
(hyperref)                setting the option has no effect on input line 1369.

) (/usr/share/texmf-dist/tex/latex/oberdiek/hypcap.sty)
(/usr/share/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/share/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/share/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/share/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/share/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/share/texmf-dist/tex/latex/cleveref/cleveref.sty))

Package csquotes Warning: No multilingual support.
(csquotes)                Cannot enable multilingual quotes on input line 5.

(./main.aux) (/usr/share/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/share/texmf-dist/tex/latex/oberdiek/epstopdf-base.sty
(/usr/share/texmf-dist/tex/latex/oberdiek/grfext.sty)
(/usr/share/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/share/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/share/texmf-dist/tex/generic/oberdiek/gettitlestring.sty))<<ot1.cmap>><<o
ml.cmap>><<oms.cmap>><<omx.cmap>><<ot1tt.cmap>>

LaTeX Font Warning: Font shape `OMS/cmtt/m/n' undefined
(Font)              using `OMS/cmsy/m/n' instead
(Font)              for symbol `textbraceleft' on input line 24.

(./section/01-motivation.tex [1{/var/lib/texmf/fonts/map/pdftex/updmap/pdftex.m
ap}]) (./section/02-background.tex [2] (./code/event.json) [3 <./figures/01_Gen
eral-eps-converted-to.pdf>]
Underfull \vbox (badness 5175) has occurred while \output is active [4 <./figur
es/03_Querying-eps-converted-to.pdf>]

LaTeX Warning: Command \textordmasculine invalid in math mode on input line 38.


) (./section/03-objectives.tex [5]) (./section/04-experiments.tex [6 <./figures
/timedistribution-eps-converted-to.pdf> <./figures/spatialdistribution_colored_
cropped.png (PNG copy)>]) (./section/05-conclusions.tex
Underfull \vbox (badness 2221) has occurred while \output is active [7 <./resul
ts/RQ1.pdf>]) (./main.bbl) [8] (./main.aux
* soulpos - computing points - it may take a few seconds * (./main.upa))

LaTeX Font Warning: Some font shapes were not available, defaults substituted.

 )
(see the transcript file for additional information)</usr/share/texmf-dist/font
s/type1/public/amsfonts/cm/cmbx10.pfb></usr/share/texmf-dist/fonts/type1/public
/amsfonts/cm/cmbx12.pfb></usr/share/texmf-dist/fonts/type1/public/amsfonts/cm/c
mbx9.pfb></usr/share/texmf-dist/fonts/type1/public/amsfonts/cm/cmex10.pfb></usr
/share/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi10.pfb></usr/share/texmf-d
ist/fonts/type1/public/amsfonts/cm/cmmi6.pfb></usr/share/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmib10.pfb></usr/share/texmf-dist/fonts/type1/public/amsfo
nts/cm/cmr10.pfb></usr/share/texmf-dist/fonts/type1/public/amsfonts/cm/cmr6.pfb
></usr/share/texmf-dist/fonts/type1/public/amsfonts/cm/cmr7.pfb></usr/share/tex
mf-dist/fonts/type1/public/amsfonts/cm/cmr9.pfb></usr/share/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmsy10.pfb></usr/share/texmf-dist/fonts/type1/public/ams
fonts/cm/cmsy7.pfb></usr/share/texmf-dist/fonts/type1/public/amsfonts/cm/cmsy9.
pfb></usr/share/texmf-dist/fonts/type1/public/amsfonts/cm/cmti10.pfb></usr/shar
e/texmf-dist/fonts/type1/public/amsfonts/cm/cmtt10.pfb></usr/share/texmf-dist/f
onts/type1/public/amsfonts/cm/cmtt9.pfb></usr/share/texmf-dist/fonts/type1/publ
ic/tex-gyre/qhvr.pfb>
Output written on main.pdf (8 pages, 1075098 bytes).
Transcript written on main.log.

